Weight update in ferroelectric memristors with identical and non-identical pulses

Ferroelectric tunnel junctions (FTJs) are a class of memristor which promise low-power, scalable, field-driven analog operation. In order to harness their full potential, operation with identical pulses is targeted. In this paper, several weight update schemes for FTJs are investigated, using either non-identical or identical pulses, and with time delays between the pulses ranging from 1 us to 10 s. Experimentally, a method for achieving non-linear weight update with identical pulses at long programming delays is demonstrated by limiting the switching current via a series resistor. Simulations show that this concept can be expanded to achieve weight update in a 1T1C cell by limiting the switching current through a transistor operating in sub-threshold or saturation mode. This leads to a maximum linearity in the weight update of 86% for a dynamic range (maximum switched polarization) of 30 {\mu}C/cm2. It is further demonstrated via simulation that engineering the device to achieve a narrower switching peak increases the linearity in scaled devices to >93 % for the same range.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

